Scalable and Jointly Differentially Private Packing

We introduce an $(\epsilon, \delta)$-jointly differentially private algorithm for packing problems. Our algorithm not only achieves the optimal trade-off between the privacy parameter $\epsilon$ and the minimum supply requirement (up to logarithmic factors), but is also scalable in the sense that the running time is linear in the number of agents $n$. Previous algorithms either run in cubic time in $n$, or require a minimum supply per resource that is $\sqrt{n}$ times larger than the best possible.

==> miss-proof-time.tex <==
\section{Missing Proofs in Time Complexity}
\label{sec:miss-proof-time}
\begin{theorem}
	The algorithm will stop before $T\geq \frac{m^2\ln(m+1)}{\alpha^2}$, if $b\geq \tilde{O}(\frac{\sqrt{m}}{\alpha \epsilon})$. 
\end{theorem}
\begin{proof}
	We show this by contradiction.
	Firstly, we show that the biggest violation $s$ increases with the number of rounds $T$, specifically, $s\geq \left(\frac{T\alpha}{2m}-\frac{2m\ln(m+1)}{\alpha}\right)\frac{1}{\eta_{sum}} $ . Note that the average violation $\bar{s}$ over the  $m$ resources,  $\bar{s}\geq \sum_{t=1}^T \sum_{j\in[m]} \eta^t(-\nabla_j D(p^t))\cdot \frac{1}{\eta_{sum}m}$. We separate $\sum_{t=1}^T \sum_{j\in[m]} \eta^t(-\nabla_j D(p^t))$ into two terms,
	\begin{align}
	\begin{split}
	\label{eq:violation}
	\textstyle  \sum_{t=1}^T \sum_{j\in[m]} \eta^t(-\nabla_j D(p^t)) =\sum_{t:\eta^t\geq  \frac{\alpha}{2mb}}\sum_{j\in[m]}\eta^t(-\nabla_j D(p^t))+\sum_{t:\eta^t\leq \frac{\alpha}{2mb}}\sum_{j\in[m]}\eta^t(-\nabla_j D(p^t))\\
	\end{split}
	\end{align}
	For the first term, note that the number of rounds such that $\frac{\alpha}{b}\geq\eta^t\geq \frac{\alpha}{2mb}$ is at most $\frac{\eta_{sum}}{\alpha/2mb}=\frac{2m\ln(m+1)}{\alpha^2}$, otherwise the algorithm has stopped according to our stopping criteria. In addition, for those rounds, we have $-2mb\leq\nabla_jD(p^t)\leq b$, which means $-\nabla_jD(p^t)\geq -b$, or equivalently, $\sum_{j\in[m]}-\nabla_jD(p^t)\geq -mb$, so 
	\begin{equation}
	\textstyle \label{eq:eta1}
	\sum_{t:\eta^t\geq \frac{\alpha}{2mb}}\sum_{j\in[m]}\eta^t(-\nabla_j D(p^t))\geq \frac{2m\ln(m+1)}{\alpha^2}\cdot \frac{\alpha}{b}\cdot (-mb)=\frac{-2m^2\ln(m+1)}{\alpha} ~. 
	\end{equation}
	For the second term, note that for the remaining $T-\frac{2m\ln(m+1)}{\alpha^2}$ rounds, in each round, there exists $j$, such that $-\nabla_j D(p^t)\geq 2mb$ since $\eta^t=\frac{\alpha}{\max_{j\in[m]}{|\nabla_jD(p^t)|}}\leq \frac{\alpha}{2mb}$, suppose that $-\nabla_jD(p^t)=kmb, k\geq 2$. For the other $m-1$ dimensions $i \neq j, \nabla_i D(p^t)\leq b$, which means$\textstyle -\nabla_i D(p^t)\geq -b$, so $\sum_{i\neq j} -\nabla_j D(p^t)\geq -mb $. Summing them up together, we have  $\sum_{j\in [m]} -\nabla_j D(p^t)\geq (k-1)mb $, further more,
	\begin{equation}
	\textstyle \label{eq:eta2}
	\sum_{t:\eta^t\leq  \frac{\alpha}{2mb}}\sum_{j\in[m]}\eta^t(-\nabla_j D(p^t))\geq (T-\frac{2m\ln(m+1)}{\alpha^2}) \cdot \frac{\alpha}{kmb}\cdot (k-1)mb\geq (T-\frac{2m\ln(m+1)}{\alpha^2})\frac{\alpha}{2} ~.
	\end{equation}
	Putting (\ref{eq:violation}), (\ref{eq:eta1}) and (\ref{eq:eta2}) together, we get that
	\begin{equation*}
	\sum_{t\in[T]} \sum_{j\in[m]} \eta^t(-\nabla_j D(p^t)) \geq \frac{-2m^2\ln(m+1)}{\alpha}+(T-\frac{2m\ln(m+1)}{\alpha^2})\frac{\alpha}{2}=\tilde{O}(\alpha T-\frac{m^2\ln(m+1)}{\alpha}) ~.
	\end{equation*}
	So $s\geq \bar{s}\geq \tilde{O}(\alpha T-\frac{m^2\ln(m+1)}{\alpha})\cdot \frac{1}{\eta_{sum} m}= \tilde{O}\left(\left(\frac{\alpha T}{m}-\frac{m\ln(m+1)}{\alpha}\right)\frac{1}{\eta_{sum}}\right)$.\\
	By lemma \ref{lemma:l(xt,pt)-l(xt,p)}, we know that 
	\begin{align*}
	\textstyle
	\sum_{t=1}^T\eta^t \left((1+\alpha)L(x^t,p^t)-L(x^t,p)\right)\leq D_{KL}(p||p^1)+\tilde{O}(\frac{\eta_{sum}\sqrt{mT}}{b\alpha\epsilon})+\eta_{sum}\tilde{O}(\alpha n) ~.\\
	\end{align*}
	For LHS, recall (\ref{eq:LHS of l(x,p)}) in \ref{subsec:feasibility}, we have 
	\begin{align*}
	\textstyle
	\sum_{t=1}^T\eta^t \left((1+\alpha)L(x^t,p^t)-L(x^t,p)\right)\geq\eta_{sum}sp_{max}\cdot\frac{1}{2}\geq  \tilde{O}\left(p_{max}\left(\frac{T\alpha}{m}-\frac{m\ln(m+1)}{\alpha}\right)\right) ~.
	\end{align*}
	So we have:
	\begin{equation}
	\label{eq:contradiction}
	\textstyle
	\tilde{O}\left(p_{max}\left(\frac{T\alpha}{m}-\frac{m\ln(m+1)}{\alpha}\right)\right)\leq D_{KL}(p||p^1)+\tilde{O}(\frac{\eta_{sum}\sqrt{mT}}{b\alpha\epsilon})+\eta_{sum}\tilde{O}(\alpha n) ~.
	\end{equation}
	We will show that there is a contradiction of (\ref{eq:contradiction}) if $T\geq \frac{m^2\ln(m+1)}{\alpha^2}$.
	
	$T\geq \frac{m^2\ln(m+1)}{\alpha^2}$ derives that $\frac{T\alpha}{2}\geq\frac{2m\ln(m+1)}{\alpha}$ and $LHS=p_{max}\tilde{O}\left(\frac{\alpha T}{m}\right)\geq \tilde{O}\left(\frac{p_{max}m\ln(m+1)}{\alpha\epsilon}\right)=\tilde{O}\left(\frac{nm\ln(m+1)}{b\alpha\epsilon}\right)$. Then we will show that the LHS of (\ref{eq:contradiction}) is larger than the RHS by showing that LHS is larger than the three terms in RHS separately.\\
	For the first term in RHS, it's obvious that $\tilde{O}\left(\frac{p_{max}m\ln(m+1)}{\alpha\epsilon}\right)\geq D_{KL}(p||p^1)=p_{max}\ln(m+1) $.\\
	For the second term in RHS,
	\begin{align*}
	p_{max}\tilde{O}\left(\frac{T\alpha}{m}\right)-\tilde{O}\left(\frac{\eta_{sum}\sqrt{mT}}{b\alpha \epsilon}\right)& \textstyle =\tilde{O}\left(\frac{\alpha nT}{bm}\right)-\tilde{O}\left(\frac{\ln(m+1)\sqrt{mT}}{\alpha^2b^2\epsilon}\right)\\
	& \textstyle =\tilde{O}\left(\frac{\sqrt{\alpha T}}{bm}\left( n\sqrt{T}-\frac{m\ln(m+1)\sqrt{m}}{\alpha^3b\epsilon}\right)\right)\\
	& \textstyle \geq \tilde{O}\left(\frac{\sqrt{T}}{bm}\left(n\sqrt{T}-\frac{m\ln(m+1)}{\alpha^2}\right)\right) \\
	& \textstyle \geq \tilde{O}\left(\frac{\sqrt{T}}{bm}\left(\frac{b m\sqrt{\ln(m+1)}}{\alpha}-\frac{m\ln(m+1)}{\alpha^2}\right)\right)\\
	& \textstyle \geq \tilde{O}\left(\frac{\sqrt{T\ln(m+1)}m}{\alpha b m}\left(b-\frac{\sqrt{\ln(m+1)}}{\alpha}\right)\right)\
	& \textstyle \geq 0 ~.
	\end{align*}
	The third and last lines follow by $b\geq \tilde{O}(\frac{\sqrt{m}}{\alpha \epsilon})$\xue{In fact $b\geq \tilde{O}(\frac{\sqrt{\ln(m+1)}}{\alpha \epsilon})$ is enough}, and the forth line follows by our assumptions $T\geq \frac{m^2\ln(m+1)}{\alpha^2}$ and $n\geq b$.
	
	For the third term in RHS,
	\begin{align*}
	\textstyle \tilde{O}\left(p_{max} \frac{\alpha T}{m}\right)- \tilde{O}\left(\eta_{sum} \alpha n\right)  \geq \tilde{O}\left(\frac{\alpha n T}{bm}-\frac{\alpha n \ln(m+1)}{\alpha b}\right)=\tilde{O}\left(\frac{n}{b}\left(\frac{\alpha T}{m}-\ln(m+1)\right)\right)\geq 0 ~.
	\end{align*}
	So, we can see that if $T\geq \frac{m^2\ln(m+1)}{\alpha^2}$, LHS of (\ref{eq:contradiction})$\geq $ RHS of (\ref{eq:contradiction}), which is a contradiction of (\ref{eq:contradiction}).
	
\end{proof}
\begin{proof}[Proof Sketch of Lemma~\ref{lemma:l(xt,pt)-l(xt,p)}]
	We present a proof sketch of a weaker claim that the inequality holds in expectation, which captures captures the bottleneck of the analysis.
	Further showing to the stronger claim in the lemma takes a (slightly nonstandard) concentration inequality for martingales.
	See Appendix~\ref{app:???} for a complete proof of the lemma.
	
	Readers familiar with this kind of analysis will find it standard and may directly jump to the end to verify that the contribution from the variance term can be bounded given the noise scales chosen by the algorithm.
	Fix any step $t$, we have the followings:
	%
	\begin{align*}
	\eta^t \big( L(x^t, p^t) - L(x^t, p) \big)
	& 
	= \langle \eta^t \nabla D(p^t), p^t - p \rangle \\[1ex]
	&                                                
	= \E \big[ \langle \delta^t, p^t - p \rangle \big] \\
	&
	= \E \left[ \big\langle \ln \big( \tfrac{\hat{p}^{t+1}}{p^t} \big), p - p^t \big\rangle \right] \\
	&
	= \E \big[ \kl\big(p\|p^t\big) - \kl\big(p\|\hat{p}^{t+1}\big) + \kl\big(p^t\|\hat{p}^{t+1}\big) \big] \\[1ex]
	&
	\le \E \big[ \kl\big(p\|p^t\big) - \kl\big(p\|p^{t+1}\big) + \kl\big(p^t\|\hat{p}^{t+1}\big) - \kl\big(p^{t+1}\|\hat{p}^{t+1}\big) \big] \\[1ex]
	&
	\le \E \big[ \kl\big(p\|p^t\big) - \kl\big(p\|p^{t+1}\big) + \kl\big(p^t\|\hat{p}^{t+1}\big) \big]
	~.
	\end{align*}
	
	We abuse notation and let $\ln\big(\frac{\hat{p}^{t+1}}{p^t}\big)$ denote a vector whose $j$-th coordinate is $\ln\big(\frac{\hat{p}^{t+1}_j}{p^t_j}\big)$ for any $j \in [m+1]$, in the 4th line of the above equation.
	The last two inequalities follow by the generalized Pythagorean theorem and the non-negativity of divergences, respectively.
	
	Summing over $t \in [T]$, the first two terms form a telescopic sum; 
	it is bounded by the first term on the right-hand-side of the inequality stated in the lemma.
	For last term, we have:
	%
	\begin{align*}
	\E \big[ \kl\big(p^t\|\hat{p}^{t+1}\big) \big]
	&
	\textstyle
	= \E \big[ \sum_{j=1}^{m+1} \big( p^t_j \ln\big(\tfrac{p^t_j}{\hat{p}^{t+1}_j}\big) - p^t_j + \hat{p}^{t+1}_j \big) \big] \\
	& 
	\textstyle
	= \E \big[ \sum_{j=1}^{m+1} p^t_j \big( \delta^t_j - 1 + \exp\big(-\delta^t_j\big) \big) \big] \\
	&
	\textstyle
	\le \E \big[ \sum_{j=1}^{m+1} p^t_j \big( \delta^t_j \big)^2 \big]
	= \sum_{j=1}^{m+1} p^t_j \big( \E \big[ \delta^t_j \big]^2 + \Var \big[ \delta^t_j \big] \big)
	~.
	\end{align*}
	
	Note that the step sizes ensure $\E \big[ \delta^t_j \big] \le \alpha$.
	The first part on the right-hand-side sums to:
	%
	\begin{align*}
	\textstyle
	\sum_{j=1}^{m+1} \sum_{t=1}^T p^t_j \cdot \E \big[ \delta^t_j \big]^2
	&    
	\textstyle
	\le \alpha \sum_{j=1}^{m+1} p^t_j \cdot \sum_{t=1}^T \big| \E \big[ \delta^t_j \big] \big| \\
	&
	\textstyle
	\le \alpha \sum_{j=1}^{m+1} p^t_j \cdot \bigg( 2b \sum_{t=1}^T \eta^t - \sum_{t=1}^T \eta^t \E \big[ \delta^t_j \big] \bigg) \\
	&
	\textstyle
	= \etasum \cdot O(\alpha n) - \alpha \sum_{j=1}^{m+1} p^t_j \sum_{t=1}^T \eta^t \E \big[ \delta^t_j \big] \\[1ex]
	&
	\textstyle
	\le \etasum \cdot O(\alpha n) - \alpha \sum_{j=1}^{m+1} p^t_j \sum_{t=1}^T \eta^t \nabla_j D(p^t) \\
	&
	\textstyle
	= \etasum \cdot O(\alpha n) - \alpha \sum_{j=1}^{m+1} \eta^t \bigg( L(x^t, p^t) - \sum_{i=1}^n v_i x^t_i \bigg) \\
	&
	\textstyle
	\le \etasum \cdot O(\alpha n) - \alpha \sum_{j=1}^{m+1} \eta^t L(x^t, p^t)
	\le \etasum \cdot O(\alpha n) 
	~.
	\end{align*}
	
	Finally, the contribution from the variance part sums to:
	%
	\begin{align*}
	\textstyle
	\sum_{j=1}^{m+1} \sum_{t=1}^T p^t_j \cdot \Var \big[ \delta^t_j \big] 
	&
	\textstyle
	\le \sum_{j=1}^{m+1} \sum_{t=1}^T p^t_j \cdot 4 \big(\sigma^t\big)^2
	&& 
	\textrm{(Lemma~\ref{lem:noise-distributions-privacy})} \\
	&
	\textstyle
	\le O \big( \sum_{t=1}^T \frac{\pmax m \etasum \eta^t}{\epsilon^2} \big) 
	&&
	\textrm{(Definition of $\sigma^t$'s)} \\
	&
	\textstyle
	\le O \big( \frac{\pmax m \etasum^2}{\epsilon} \big) \\
	&
	\textstyle
	= \etasum \cdot \tilde{O} \big( \frac{n}{\alpha \epsilon^2 b^2} \big) \le \etasum \cdot O(\alpha n)
	~.
	&&
	\textrm{(Assumption on $b$)}
	\end{align*}
	
	Putting together proves the lemma.
\end{proof}



\begin{comment}
\begin{theorem}
\label{thm:martingale-concentration}
Suppose $X^1, X^2, \dots, X^T$ is a martingale w.r.t.\ $r^1, r^2, \dots, r^T$ such that $|X^t - X^{t-1}| \le 1$ for any $t \in [T]$ (with $X^0 = 0$), and that:
%
\[
\sum_{t = 1}^T \Var \big[ X^t ~\big|~ r^{1:t-1} \big] \le \sigma^2 ~.
\]
%
Then, we have that:
%
\xue{here, I think (1) should be labled on the above equation when used in the proof}
\begin{equation}
\label{eqn:martingale-bounded-total-variance}
\Pr \big[ X^T \ge \alpha \big] \le \exp \big( - \frac{\alpha^2}{4 \sigma^2} \big) 
~.
\end{equation}
\end{theorem}
We include the proof of the above two lemmas in Appendix \ref{sec:miss-proof-utility} for sake of completeness. In addition, we have the following lemma whose proof is also deferred to Appendix \ref{sec:miss-proof-utility}  .
\begin{lemma}
\label{lemma:l(xt,pt)-opt}
$$\sum_{t\in[T]} \eta_t L(x^t,p^t)\geq \sum_{t\in [T]}\eta_t \sum_{i\in[n]} \pi_i x^{*}_i =OPT\cdot \eta_{sum}~.$$
\end{lemma}
\end{comment}


